Trusting Your AI Agent Emotionally and Cognitively: Development and Validation of a Semantic Differential Scale for AI Trust

Trust is not just a cognitive issue but also an emotional one, yet the research in human-AI interactions has primarily focused on the cognitive route of trust development. Recent work has highlighted the importance of studying affective trust towards AI, especially in the context of emerging human-like LLMs-powered conversational agents. However, there is a lack of validated and generalizable measures for the two-dimensional construct of trust in AI agents. To address this gap, we developed and validated a set of 27-item semantic differential scales for affective and cognitive trust through a scenario-based survey study. We then further validated and applied the scale through an experiment study. Our empirical findings showed how the emotional and cognitive aspects of trust interact with each other and collectively shape a person's overall trust in AI agents. Our study methodology and findings also provide insights into the capability of the state-of-art LLMs to foster trust through different routes.

==> 0-0-tables-and-figures.tex <==
\newcommand{\tableValB}{\begin{table}[]
\caption{Linear regression models predicting the two final scales from the manipulation and control variables. Model 1 shows the effects on the affective trust scale, Model 2 shows the effects on the cognitive trust scale, and Model 3 shows the effects of both scales on general trust.}
\label{tab:table-val-b}
\begin{tabular}{llll}
\hline
      & \textbf{Model 1}      & \textbf{Model 2}        & \textbf{Model 3} \\ \cline{2-4} 
                        & Affective Trust Scale & Cognitive   Trust Scale & General Trust    \\
                        & Coef. (S.E.)          & Coef. (S.E.)            & Coef. (S.E.)     \\ \hline
Affective   Trust Scale & /                     & /                       & \cellcolor{lightgray} 0.502   (0.227)* \\
Cognitive Trust Scale   & /                     & /                       & \cellcolor{mediumgray} 0.864 (0.256)**  \\
Low Affective Trust     & -0.291   (0.311)      & 0.198   (0.276)         & 0.149   (0.390)  \\
Low Cognitive Trust     & 0.252   (0.329)       & \cellcolor{mediumgray} -0.857   (0.292)** & -0.217   (0.477) \\
Low Affective Trust x Low Cognitive Trust & \cellcolor{darkgray} -1.939   (0.448)*** & \cellcolor{mediumgray} -1.257   (0.397)** & 0.251   (0.609)  \\
Age                     & -0.004   (0.008)      & -0.012   (0.007)        & 0.006   (0.010)  \\
AI Familiarity          & -0.029   (0.106)      & 0.047   (0.094)         & 0.149   (0.129)  \\
AI Literacy             & \cellcolor{lightgray} 0.153   (0.071)*      & -0.003   (0.063)        & -0.054   (0.092) \\
Trust Disposition       & 0.114   (0.080)       & 0.092   (0.071)         & -0.064   (0.098) \\
Order of Scenario       & -0.146   (0.221)      & -0.078   (0.196)        & -0.033   (0.266) \\
Intercept               & 0.422   (0.570)       & \cellcolor{mediumgray} 1.513   (0.505)**       & \cellcolor{lightgray} 1.588   (0.756)* \\
R-squared               & 0.543                 & 0.561                   & 0.682            \\ \hline
\multicolumn{4}{r}{\textit{*p\textless{}0.05; **p\textless{}0.01; ***p\textless{}0.001}}
\end{tabular}
\end{table}
}

==> 12-ethical.tex <==
\newpage
\section{Ethical Statement}
All of the study protocols used in this work were reviewed and exempted by IRB. The scenarios used in our studies covered common use cases of AI assistants, such as providing emotional support, technical assistance, or social activity planning. We avoided using sensitive topics that could cause discomfort or distress to participants.

==> 3-related-work.tex <==
\section{Related Work}

\todo{Add affect computing literature}
\todo{Add communication, how people anthropomorphize AI and communication breaks down with low trust}

% Section 1 - Importance of affective trust
% Importance of aff and cog trust in human-human context, later connect back to why they manifest in an AI context

The human trust literature has shown that affective and cognitive trust has different impacts on interpersonal relationships \cite{webber2008development, mcallister1995affect}. While cognitive trust can be more quickly constructed \cite{mcknight2002impact, meyerson1996swift}, affective trust is more persistent under challenges in teamwork \cite{mcallister1995affect} and interpersonal relationships \cite{williams2001whom}. Once developed, affective trust is also more resistant, allowing for short-term problems and mistakes \cite{jones1998experience, mcallister1995affect}. Studies in psychology, neurology, and computer science have demonstrated the importance of psychological influence (e.g., emotions, personality, moods) on the decision-making process \cite{nunes2012personalityml}. Researchers argued that affective and cognitive trust complement each other \cite{granatyr2017need}, since affective trust needs to be developed on the basis of cognitive trust \cite{johnson2005cognitive}. 

% Importance of studying aff and cog trust in the human-AI context
Prior work has shown that similar to trust towards humans, trust towards technology has both cognitive and affective components \cite{komiak2004understanding}. Cognitive trust is defined as the user's intellectual perceptions of the system's characteristics, while affective trust is defined as people's emotional responses to the system \cite{madsen2000measuring, ueno2022trust}. In trust towards AI, emotional and cognitive trust serve different functions: dimensions of emotional trust include tangibility, anthropomorphism and immediacy behaviors, while dimensions of cognitive trust include tangibility, transparency, reliability, task characteristics and immediacy behaviors \cite{glikson2020human}. In the realm of Human-Robot Interaction (HRI), trust has also been investigated through dual-dimensional models. Law and Scheutz \cite{law2021trust} differentiated between Performance-based (P) trust, focusing on a robot's reliability and competence, and Relation-based (R) trust, emphasizing trust in a robot as a social entity. Similarly, Malle and Ullman's Multi-Dimensional Measure of Trust (MDMT) model \cite{malle2021multidimensional} identifies Performance trust (encompassing Reliability and Capability) and Moral trust (incorporating Sincerity and Ethical aspects). While these models is similar to the Cognitive-Affective (C-A) trust model in their bidimensional structure, they do not fully capture the complexities of emotional aspects of trust, especially given the enhanced affective capability brought by Large Language Model that opens up opportunities for relationship building with AI agents.

%\textcolor{blue}{In the domain of Human-Robot Interaction (HRI), trust has been examined through two-dimensional models. Law and Scheutz \cite{law2021trust} explored the dichotomy, defining Performance-based (P) trust as the robot's reliability and competence, and Relation-based (R) trust as the robot's ability to be trusted as a social agent. The Multi-Dimensional Measure of Trust (MDMT) model proposed by Malle and Ullman \cite{malle2021multidimensional} also captures two underlying factors of trust: Performance trust and Moral trust, where Performance trust includes Reliable and Capable dimensions, and Moral trust includes Sincere and Ethical dimensions. While the P-R trust and the MDMT model share similarities with the Cognitive-Affective (C-A) trust model, particularly in their dual-dimensional approach that differentiates between a system's functional performance and social aspects, it may not fully encapsulate the intricacies inherent in AI advisors. These AI systems engage deeply with psychological facets of trust, which are more comprehensively captured by the C-A model. Thus, our work focuses on the C-A model that provides a more nuanced framework for understanding trust in AI advisors.}

% Importance of affective trust

While most prior work on trust in AI is focused on cognitive trust, affective trust is crucial for the adoption of a complex new technology like AI. The unknown complexity of AI suggests a need for a ``leap of faith" and trust in its hidden processes that cannot be directly observed or cognitively understood \cite{hoff2015trust, lee2004trust}. Cognitive trust alone is inadequate to account for how people actually make decisions upon trust, rational choice overstates people's cognitive capacities to fully comprehend the decision of a complex system \cite{komiak2006effects}. For example, researchers have shown that even with additional support through explanations, people are still not able to detect AI's inaccurate recommendations \cite{jacobs2021machine, buccinca2021trust}. Granatyr et al. \cite{granatyr2017need} have provided a theoretical foundation for the importance of exploring affective factors of trust in AI systems beyond the traditional numeric and cognitive paradigm. A few recent works have highlighted that affect-based trust plays a decisive role in people's acceptance of AI-based technology in preventative health interventions \cite{kyung2022rationally} and financial services robo-advising \cite{zhang2021you}. Research in explainable AI (XAI) has also shown that people's affective responses to explanations are crucial in improving personalization and increasing trust in AI systems \cite{guerdan2021toward}. 

% Measurements used in human trust lit are not generalizable to AI

Different models and measurements have been established in the human trust literature, including Hoff and Bashir's three-layered trust model (benevolence, integrity, and ability) \cite{hoff2015trust}, Madsen and Gregor's Model of Human-Computer Trust \cite{madsen2000measuring}, and Johnson and Grayson's model in service relationship \cite{johnson2005cognitive}. However, the validity of those scales was not examined in the context of humans interacting with an AI agent. The following problems with prior work's usage of the scales have been identified: First, trust items were adopted directly from a human trust context to measure affective trust in AI with minor changes in word choice. The set of items might not be generalizable to AI assistants. For example, the trust items developed for Human-Computer Trust were directly used to measure affective trust for an AI system collecting personal information \cite{liao2021should}. In addition, there is a lack of consensus on what constitutes affective trust when the models are adopted. For example, while Kyung and Kwon merged the benevolence and integrity dimensions of the three-layered trust model to measure affective trust towards AI-based preventive health interventions \cite{kyung2022rationally}, Shi et al. \cite{shi2021antecedents} categorized all three dimensions as cognitive trust and adopted a different scale \cite{komiak2006effects} for affective trust. Under the general need to create a uniform and valid measure of trust for AI-based technologies \cite{ueno2022trust}, our work looks specifically at measures of affective trust in human-AI interaction. 

% Semantic differentials

Most pre-existing questionnaires measuring trust are using Likert-type scales. In this work, we followed Verhagen et al.'s framework to develop semantic differential scales for affective and cognitive trust in AI \cite{verhagen2015toward}. Semantic differentials present respondents with a set of bipolar adjective items in antonym pairs. Semantic differentials have the advantage over Likert-style items since respondents' selection of the option ``Strongly disagree" does not necessarily imply that the respondent agrees with the opposite of the item \cite{chin2008fast}. Semantic differentials can reduce acquiescence bias, which refers to the response biases that result from participants having a tendency to agree with all items or indicate a positive connotation \cite{friborg2006likert}. Semantic differentials have been shown to outperform Likert-based scaling on robustness \cite{hawkins1974stapel}, reliability \cite{wirtz2003examination}, and validity \cite{van1995assessment}.

==> figures/figure-gpt-definition.tex <==
\begin{comment}
%%% ChatGPT's definition of Affective and Cognitive Trust
\begin{figure*}
    \centering
    \includegraphics[width=0.6\linewidth]{chatgpt-def.png}
    \caption{Screenshot of ChatGPT's responses to the definitions of affective and cognitive trust.}
    \label{fig:chatgpt-def}
    \Description{Screenshot of ChatGPT's responses to the definitions of affective and cognitive trust.}
\end{figure*}
\end{comment}

==> tables/table-1-items-all-v1.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table*}[]
\setuptable
\caption{The table displays the initial set of 33 items for cognitive and affective trust in the form of antonym pairs before the elimination process through exploratory factor analysis. The ``All" and ``AI condition" columns show the final items and their factor loadings with respect to 1) all data and 2) the subset of data under the AI agent condition. This shows that the items and the two-factor structure is also consistent when we conducted the same exploratory factor analysis for only the AI agent condition. The columns F1 and F2 show the items' factor loadings on each factor. The empty rows correspond to the eliminated items.}
\label{tab:items}
\begin{tabular}{llllllll}
 &
   &
   &
  All &
   &
  AI Condition &
   &
   \\ \hline
\# &
  Item &
  Sub-dimension &
  F1 &
  F2 &
  F1 &
  F2 &
  Source \\ \hline
C1 &
  Unreliable - Reliable &
  Reliability &
  0.905 &
  0 &
  0.922 &
  -0.058 &
  \cite{mcallister1995affect,johnson2005cognitive,erdem2003cognitive,madsen2000measuring,gefen2002reflections} \\
C2 &
  Inconsistent - Consistent &
   &
  0.928 &
  -0.12 &
  0.924 &
  -0.183 &
  \cite{mcallister1995affect,johnson2005cognitive,erdem2003cognitive,madsen2000measuring} \\
C3 &
  Unpredictable - Predictable &
   &
  0.894 &
  -0.171 &
  0.898 &
  -0.204 &
  \cite{madsen2000measuring} \\
C4 &
  Undependable - Dependable &
   &
  0.851 &
  0.016 &
  0.911 &
  -0.111 &
  \cite{mcallister1995affect,johnson2005cognitive,erdem2003cognitive,madsen2000measuring} \\
C5 &
  Fickle - Dedicated &
   &
  0.759 &
  0.139 &
  0.744 &
  0.116 &
  \cite{mcallister1995affect,johnson2005cognitive,madsen2000measuring} \\
C6 &
  Careless - Careful &
   &
  0.721 &
  0.213 &
  0.716 &
  0.206 &
  \cite{mcallister1995affect,johnson2005cognitive} \\
C7 &
  Unbelievable - Believable &
   &
  0.69 &
  0.082 &
  0.658 &
  0.034 &
  \cite{erdem2003cognitive,madsen2000measuring,gefen2002reflections} \\
C8 &
  Unpromising - Promising &
   &
   &
   &
   &
   &
  \cite{erdem2003cognitive,madsen2000measuring,gefen2002reflections} \\
C9 &
  Clueless - Knowledgable &
  Competence &
  0.907 &
  -0.018 &
  0.898 &
  0.026 &
  \cite{komiak2006effects,madsen2000measuring,gefen2002reflections} \\
C10 &
  Incompetent - Competent &
   &
  0.9 &
  0.023 &
  0.921 &
  -0.021 &
  \cite{mcallister1995affect,johnson2005cognitive,komiak2006effects,madsen2000measuring,gefen2002reflections} \\
C11 &
  Ineffective - Effective &
   &
  0.861 &
  0.075 &
  0.863 &
  0.071 &
  \cite{madsen2000measuring,gefen2002reflections} \\
C12 &
  Inexperienced - Experienced &
   &
  0.751 &
  0.089 &
  0.611 &
  0.155 &
  \cite{mcallister1995affect,johnson2005cognitive,komiak2006effects,gefen2002reflections} \\
C13 &
  Amateur - Proficient &
  Understandability &
  0.895 &
  0.009 &
  0.864 &
  0.039 &
  \cite{mcallister1995affect,johnson2005cognitive,erdem2003cognitive,komiak2006effects,madsen2000measuring,gefen2002reflections} \\
C14 &
  Irrational - Rational &
   &
  0.827 &
  0.02 &
  0.792 &
  0.05 &
  \cite{madsen2000measuring,gefen2002reflections} \\
C15 &
  Unreasonable - Reasonable &
   &
  0.71 &
  0.224 &
  0.714 &
  0.202 &
  \cite{madsen2000measuring,gefen2002reflections} \\
C16 &
  Incomprehensible - Understandable &
   &
  0.706 &
  0.175 &
  0.783 &
  0.079 &
  \cite{komiak2006effects,madsen2000measuring} \\
C17 &
  Opaque - Transparent &
   &
  0.6 &
  0.261 &
  0.656 &
  0.18 &
  \cite{erdem2003cognitive,komiak2006effects,madsen2000measuring} \\
C18 &
  Dishonest - Honest &
  Integrity &
  0.693 &
  0.178 &
  0.743 &
  0.097 &
  \cite{erdem2003cognitive,komiak2006effects,gefen2002reflections} \\
C19 &
  Unfair - Fair &
   &
  0.663 &
  0.274 &
  0.66 &
  0.268 &
  \cite{erdem2003cognitive,komiak2006effects} \\
C20 &
  Insincere - Sincere &
   &
   &
   &
   &
   &
  \cite{komiak2006effects,gefen2002reflections} \\ \hline
A1 &
  Apathetic - Empathetic &
  Benevolence &
  -0.11 &
  0.989 &
  -0.162 &
  0.967 &
  \cite{mcallister1995affect,johnson2005cognitive} \\
A2 &
  Insensitive - Sensitive &
   &
  -0.08 &
  0.959 &
  -0.109 &
  0.955 &
  \cite{mcallister1995affect,johnson2005cognitive,erdem2003cognitive} \\
A3 &
  Impersonal - Personal &
   &
  -0.024 &
  0.902 &
  -0.025 &
  0.847 &
  \cite{johnson2005cognitive,erdem2003cognitive,madsen2000measuring} \\
A4 &
  Ignoring - Caring &
   &
  0.048 &
  0.881 &
  -0.055 &
  0.941 &
  \cite{mcallister1995affect,johnson2005cognitive,erdem2003cognitive} \\
A5 &
  Self-serving - Altruistic &
   &
  0.215 &
  0.627 &
  0.207 &
  0.622 &
  \cite{johnson2005cognitive,erdem2003cognitive,gefen2002reflections} \\
A6 &
  Malicious - Benevolent &
   &
   &
   &
   &
   &
  \cite{komiak2006effects,gefen2002reflections} \\
A7 &
  Harmful - Well-intentioned &
   &
   &
   &
   &
   &
  \cite{komiak2006effects,gefen2002reflections} \\
A8 &
  Discouraging - Supportive &
   &
   &
   &
   &
   &
  \cite{erdem2003cognitive,komiak2006effects,gefen2002reflections} \\
A9 &
  Rude - Cordial &
  Amiability &
  -0.11 &
  0.989 &
  0.112 &
  0.76 &
  \cite{mcallister1995affect,johnson2005cognitive} \\
A10 &
  Indifferent - Responsive &
   &
  0.221 &
  0.711 &
  0.232 &
  0.667 &
  \cite{mcallister1995affect,johnson2005cognitive,erdem2003cognitive,komiak2006effects,gefen2002reflections} \\
A11 &
  Judgemental - Open-minded &
   &
  0.142 &
  0.688 &
  0.078 &
  0.697 &
  \cite{erdem2003cognitive} \\
A12 &
  Impatient - Patient &
   &
  0.291 &
  0.577 &
  0.218 &
  0.6 &
  \cite{mcallister1995affect,johnson2005cognitive} \\
A13 &
  Unpleasant - Likable &
   &
   &
   &
   &
   &
  \cite{komiak2006effects,madsen2000measuring}
\end{tabular}
\end{table*} 
